Unsupervised Representation Learning of Complex Time Series for Maneuverability State Identification in Smart Mobility

Multivariate Time Series (MTS) data capture temporal behaviors to provide invaluable insights into various physical dynamic phenomena. In smart mobility, MTS plays a crucial role in providing temporal dynamics of behaviors such as maneuver patterns, enabling early detection of anomalous behaviors while facilitating pro-activity in Prognostics and Health Management (PHM). In this work, we aim to address challenges associated with modeling MTS data collected from a vehicle using sensors. Our goal is to investigate the effectiveness of two distinct unsupervised representation learning approaches in identifying maneuvering states in smart mobility. Specifically, we focus on some bivariate accelerations extracted from 2.5 years of driving, where the dataset is non-stationary, long, noisy, and completely unlabeled, making manual labeling impractical. The approaches of interest are Temporal Neighborhood Coding for Maneuvering (TNC4Maneuvering) and Decoupled Local and Global Representation learner for Maneuvering (DLG4Maneuvering). The main advantage of these frameworks is that they capture transferable insights in a form of representations from the data that can be effectively applied in multiple subsequent tasks, such as time-series classification, clustering, and multi-linear regression, which are the quantitative measures and qualitative measures, including visualization of representations themselves and resulting reconstructed MTS, respectively. We compare their effectiveness, where possible, in order to gain insights into which approach is more effective in identifying maneuvering states in smart mobility.

==> experiments.tex <==
\section{Experiments} \label{sec:enc-results}

TNC4maneuvering extends \cite{tlebese}, it is implemented in PyTorch framework (v1.12.1). Whereas DLG4Maneuvering adapted from \cite{tonekaboni2022decoupling}, it is implemented in Tensorflow framework (2.6.2). All experiments are conducted using a single Nvidia Tesla P40 GPU with CUDA 11.2.152. In our dataset, we only apply normalization as a pre-processing stage to avoid statistical biases that can lead to misinterpretation of the encoded results, unlike in the works of \cite{sajal2019cost} where a (Debauches) wavelet filtering was applied in order to remove high frequency noise on signals via denoising. \\ 

Vehicle maneuvering is an automotive problem that is central to understanding driving behavior from sensory signals. Our use-case vehicle is a Peugeot 208 model used as a fleet car, where operation time is accumulated as an amount of time where driving activities are collected by different sensors. In this particular work we focus only on the two accelerations, namely the lateral $(a_{lat})$ which is the effective measure of cornering (negative is for right turning, $0$ is straight line or breaking and positive is left turning) and the longitudinal acceleration $(a_{lon})$ where the straight line acceleration (negative braking, $0$ is constant speed and positive is accelerating). Both accelerations are reported as a fraction of the gravitational acceleration (ms$^{-2}$). Both inputs are normalized such that each $X_i = x_i/x_{\max} \in [-1, 1]$, for $x_{\max} = \max|x_i|, i = \{1, 2\}$, preserving the zero values on each feature. Here we only consider one bivariate sample signal with signal lengths 1957, with covered time of 584 minutes and mileage of 20 kilometers as shown in figure \ref{fig:reps_vis} (excluding the reconstruction parts in green color).

% From All evaluations results are based on results from include three downstream tasks: clustering, classification, and multi-linear regression. % and the source code is available on GitHub\footnote{\url{https://github.com/ThabangDLebese/tnc4maneuvering}}. 
